Secure and Efficient $L^p$-Norm Computation for Two-Party Learning Applications

Secure norm computation is becoming increasingly important in many real-world learning applications. However, existing cryptographic systems often lack a general framework for securely computing the $L^p$-norm over private inputs held by different parties. These systems often treat secure norm computation as a black-box process, neglecting to design tailored cryptographic protocols that optimize performance. Moreover, they predominantly focus on the $L^2$-norm, paying little attention to other popular $L^p$-norms, such as $L^1$ and $L^\infty$, which are commonly used in practice, such as machine learning tasks and location-based services. To our best knowledge, we propose the first comprehensive framework for secure two-party $L^p$-norm computations ($L^1$, $L^2$, and $L^\infty$), denoted as \mbox{Crypto-$L^p$}, designed to be versatile across various applications. We have designed, implemented, and thoroughly evaluated our framework across a wide range of benchmarking applications, state-of-the-art (SOTA) cryptographic protocols, and real-world datasets to validate its effectiveness and practical applicability. In summary, \mbox{Crypto-$L^p$} outperforms prior works on secure $L^p$-norm computation, achieving $82\times$, $271\times$, and $42\times$ improvements in runtime while reducing communication overhead by $36\times$, $4\times$, and $21\times$ for $p=1$, $2$, and $\infty$, respectively. Furthermore, we take the first step in adapting our Crypto-$L^p$ framework for secure machine learning inference, reducing communication costs by $3\times$ compared to SOTA systems while maintaining comparable runtime and accuracy.

==> commands.tex <==
\makeatletter
\newcommand{\multio}[1]{%
  \begin{tabularx}{\dimexpr\linewidth+\algorithmicindent}[t]{@{}X@{}}
    #1
  \end{tabularx}
}
\makeatother
\newcommand{\Input}[1]{%
  \Statex \hspace*{-\algorithmicindent}\multio{\textbf{Input: } #1}%
}
\newcommand{\Output}[1]{%
  \Statex \hspace*{-\algorithmicindent}\multio{\textbf{Output: } #1}%
}
\makeatletter
\newcommand{\multiline}[1]{%
  \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    #1
  \end{tabularx}
}
\makeatother
\newcommand{\eq}[1]{\text{eq}_{#1}}
\newcommand{\lt}[1]{\text{lt}_{#1}}
\newcommand{\share}[1]{\langle{#1}\rangle}
\newcommand{\ashare}[2]{\langle{#1}\rangle^{#2}}
\newcommand{\bshare}[1]{\langle{#1}\rangle^B}
\newcommand{\yshare}[1]{\langle{#1}\rangle^Y}
\newcommand{\func}[2]{\mathcal{F}_{\text{#1}}^{#2}}
\newcommand{\iknp}{\cite{goos_extending_2003,asharov_more_2013,kolesnikov_improved_2013,keller_actively_2015}}
\newcommand{\vole}{\cite{boyle_efficient_2019,boyle_efficient_2019-1,schoppmann_distributed_2019,geoffroy_silver_2021,yang_ferret_2020}}
\newcommand{\addernet}{\cite{you_shiftaddnet_2020,xu_kernel_2020,addernet}}
\newcommand{\etal}[1]{#1 et al.}
\makeatletter
\newcommand*{\ov}[1]{%
  \m@th\overline{\raisebox{0pt}[0.85\height]{#1}}%
}
\makeatother
\renewcommand{\algorithmiccomment}[1]{\hfill\textcolor[rgb]{0.42, 0.58, 0.34}{$\triangleright$ #1}}
\newcommand\doubleplus{\kern-0.6ex+\kern-1.3ex+}

\newcommand{\tick}{\ding{51}}
\newcommand{\cross}{\ding{55}}

\newcommand{\sys}{\mbox{Crypto-$L^p$}\xspace}

%  Feedback Tools
\newcommand{\YH}[1]{\textcolor{blue}{[YH: ~#1]}}
\newcommand{\LWR}[1]{\noindent \textcolor{pink}{[\textbf{LWR}: ~#1]}}
\newcommand{\alarst}[1]{\noindent \textcolor{blue}{[\textbf{ALRST}: ~#1]}}
\newcommand{\todo}[1]{\noindent \textcolor{red}{[\textbf{TODO}: ~#1]}}
\newcommand{\hl}[2][red]{\textcolor{#1}{#2}}
\newcommand{\BY}[1]{\textcolor{brown}{[BY: ~#1]}}
\newcommand{\JL}[1]{\noindent\textcolor{magenta}{[JL: ~#1]}}

